Neural Neighbor Style Transfer

We propose Neural Neighbor Style Transfer (NNST), a pipeline that offers state-of-the-art quality, generalization, and competitive efficiency for artistic style transfer. Our approach is based on explicitly replacing neural features extracted from the content input (to be stylized) with those from a style exemplar, then synthesizing the final output based on these rearranged features. While the spirit of our approach is similar to prior work, we show that our design decisions dramatically improve the final visual quality.

==> Figs/giraffe.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'giraffe.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%%
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{1285.33066406bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.66496834)%
  \small
    \put(0,0){\includegraphics[width=\unitlength]{giraffe.pdf}}%
    \put(0.18517643,0.64605297){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{style}}}%
    \put(0.47633362,0.64605297){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{content}}}%
    \put(0.28812417,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{segmentation masks}}}%
    \put(0.68267279,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{Gatys et al.}}}%
    \put(0.88829473,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{Kolkin et al.}}}%
    \put(0.88780847,0.64605297){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{ours no guide}}}%
    \put(0.68287337,0.64605297){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{ours guided}}}%
  \end{picture}%
\endgroup%


==> Figs/lynx.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'lynx.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%%
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{912bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.63777969)%
    \put(0,0){\includegraphics[width=\unitlength]{lynx.pdf}}%
    \put(0.14146107,0.61630217){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{keyframe \#1}}}%
    \put(0.85899121,0.61630217){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{keyframe \#2}}}%
    \put(0.49970703,0.61630217){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{inbetween frame}}}%
    \put(0.13973924,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{NNST-Opt}}}%
    \put(0.85903749,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{NNST-Opt}}}%
    \put(0.50152652,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{Jamri\v{s}ka et al.}}}%
    \Huge
    \put(0.32017544,0.17056695){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{...}}}%
    \put(0.32017544,0.46004064){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{...}}}%
    \put(0.67982456,0.46004064){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{...}}}%
    \put(0.67982456,0.17056695){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{...}}}%
  \end{picture}%
\endgroup%


==> Figs/puffin.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'puffin.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%%
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{2811.96992188bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.31051845)%
    \put(0,0){\includegraphics[width=\unitlength]{puffin.pdf}}%
    \small
    \put(0.18178759,0.30514317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{style}}}%
    \put(0.47176405,0.30514317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{content}}}%
    \put(0.68360939,0.30514317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{NNST-Opt}}}%
    \put(0.89602821,0.34014317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{NNST-Opt +}}}%
    \put(0.89602821,0.30514317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{Texler et al.}}}%
  \end{picture}%
\endgroup%

